auditor: an R Package for Model-Agnostic Visual Validation and Diagnostics

Machine learning models have spread to almost every area of life. They are successfully applied in biology, medicine, finance, physics, and other fields. With modern software it is easy to train even a~complex model that fits the training data and results in high accuracy on the test set. The problem arises when models fail confronted with real-world data. This paper describes methodology and tools for model-agnostic audit. Introduced techniques facilitate assessing and comparing the goodness of fit and performance of models. In~addition, they may be used for the analysis of the similarity of residuals and for identification of~outliers and influential observations. The examination is carried out by diagnostic scores and visual verification. Presented methods were implemented in the auditor package for R. Due to flexible and~consistent grammar, it is simple to validate models of any classes.

==> chapters/acknowledgements.tex <==
\section{Acknowledgements}

We would like to acknowledge and thank Hubert Baniecki and Tomasz Mikołajczyk for their valuable contribution to the development of the package, especially the plots.

We would also like to thank Aleksandra \mbox{Grudziąż} and Mateusz Staniak for helpful discussions.
Also, we wish to thank Dr. Rafael De Andrade Moral for his assistance and help related to the \pkg{hnp} package. 

The work was supported by NCN Opus grant 2016/21/B/ST6/02176.

